Exploiting Fairness to Enhance Sensitive Attributes Reconstruction

In recent years, a growing body of work has emerged on how to learn machine learning models under fairness constraints, often expressed with respect to some sensitive attributes. In this work, we consider the setting in which an adversary has black-box access to a target model and show that information about this model's fairness can be exploited by the adversary to enhance his reconstruction of the sensitive attributes of the training data. More precisely, we propose a generic reconstruction correction method, which takes as input an initial guess made by the adversary and corrects it to comply with some user-defined constraints (such as the fairness information) while minimizing the changes in the adversary's guess. The proposed method is agnostic to the type of target model, the fairness-aware learning method as well as the auxiliary knowledge of the adversary. To assess the applicability of our approach, we have conducted a thorough experimental evaluation on two state-of-the-art fair learning methods, using four different fairness metrics with a wide range of tolerances and with three datasets of diverse sizes and sensitive attributes. The experimental results demonstrate the effectiveness of the proposed approach to improve the reconstruction of the sensitive attributes of the training set.

==> datasets.tex <==
\begin{table*}[hbt]
\caption{Summary of the datasets used in our experiments}
\label{tab:datasets}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Ref.}                                                       & \textbf{Dataset}                                                                         & \begin{tabular}[c]{@{}c@{}}\textbf{Binary} \\ \textbf{Prediction Task}\end{tabular}                & \textbf{\#Datapoints} & \textbf{\#Non Sensitive Features} & \textbf{Sensitive Feature}       \\ \hline
\citep{Dua:2019} & UCI Adult Income                                                                & Income above \$50K                                                               & 45,222       & 13                                                                  & Gender (Male/Female)                                               \\ \hline
\citep{DBLP:conf/nips/DingHMS21} & \begin{tabular}[c]{@{}c@{}}ACSPublicCoverage\\ (Texas State, 2018)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Coverage from public \\ health insurance\end{tabular} & 98,928       & 18                                                                  & Age (First Quartile/Others)                                         \\ \hline
\citep{DBLP:conf/nips/DingHMS21} & \begin{tabular}[c]{@{}c@{}}ACSIncome \\ (Texas State, 2018)\end{tabular}        & Income above \$50K                                                               & 135,924      & 9                                                                   & \begin{tabular}[c]{@{}c@{}}Race Code \\ (White/Other)\end{tabular} \\ \hline
\end{tabular}
\end{table*}

==> datasets_attrs_detailed.tex <==
\begin{table*}[hbt]
\caption{Summary of the datasets used in our experiments}
\label{tab:datasets}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Ref.}                    & \textbf{Dataset}                                                                & \textbf{Binary Prediction Task}                                                  & \textbf{\#Datapoints} & \textbf{\#Non Sensitive Features}                                    & \textbf{Sensitive Feature}                                         \\ \hline
\citep{Dua:2019}                 & UCI Adult Income                                                                & Income above \$50K                                                               & 45,222                & \begin{tabular}[c]{@{}c@{}}7 categorical\\ 6 numerical\end{tabular}  & Gender (Male/Female)                                               \\ \hline
\citep{DBLP:conf/nips/DingHMS21} & \begin{tabular}[c]{@{}c@{}}ACSPublicCoverage\\ (Texas State, 2018)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Coverage from public \\ health insurance\end{tabular} & 98,928                & \begin{tabular}[c]{@{}c@{}}17 categorical\\ 1 numerical\end{tabular} & Age(First Quartile/Others)                                         \\ \hline
\citep{DBLP:conf/nips/DingHMS21} & \begin{tabular}[c]{@{}c@{}}ACSIncome \\ (Texas State, 2018)\end{tabular}        & Income above \$50K                                                               & 135,924               & \begin{tabular}[c]{@{}c@{}}7 categorical\\ 2 numerical\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Race Code \\ (White/Other)\end{tabular} \\ \hline
\end{tabular}
\end{table*}

==> metrics.tex <==
\begin{table*}[hbt]
\caption{Summary of the considered statistical fairness metrics}
\label{tab:metrics}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Ref.}                                          & \textbf{Metric  }            & \textbf{Equalized Measure}                                \\ \hline
\citep{dwork2012fairness}    & Statistical Parity  & Probability of being assigned the positive class \\ \hline
\citep{chouldechova2017fair} & Predictive Equality & False Positive Rate                              \\ \hline
\citep{hardt2016equality}    & Equal Opportunity   & True Positive Rate                               \\ \hline
\citep{hardt2016equality}    & Equalized Odds      & False Positive Rate and True Positive Rate       \\ \hline
\end{tabular}
\end{table*}

==> metrics_with_expression.tex <==
\begin{table*}[hbt]
\caption{Summary of the considered statistical fairness metrics}
\label{tab:metrics}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Ref.}                & \textbf{Metric}     & \textbf{Equalized Measure}                 & \textbf{Constraint Expression}                                                                                                                                                   \\ \hline
\citep{dwork2012fairness}    & Statistical Parity  & Probability of positive prediction         & $\forall \onesensattr,~ \lvert \mathbb{P}(\oneprediction = 1) - \mathbb{P}(\oneprediction = 1 \mid \onesensattr) \rvert \leq \tol$                                               \\ \hline
\citep{chouldechova2017fair} & Predictive Equality & False Positive Rate                        & $\forall \onesensattr,~ \lvert \mathbb{P}(\oneprediction = 1 \mid \onegroundtruth = 0) - \mathbb{P}(\oneprediction = 1 \mid \onesensattr,~\onegroundtruth = 0) \rvert \leq \tol$ \\ \hline
\citep{hardt2016equality}    & Equal Opportunity   & True Positive Rate                         & $\forall \onesensattr,~ \lvert \mathbb{P}(\oneprediction = 1 \mid \onegroundtruth = 1) - \mathbb{P}(\oneprediction = 1 \mid \onesensattr,~\onegroundtruth = 1) \rvert \leq \tol$ \\ \hline
\citep{hardt2016equality}    & Equalized Odds      & False Positive Rate and True Positive Rate & Conjunction of Predictive Equality and Equal Opportunity                                                                                                                         \\ \hline
\end{tabular}
\end{table*}

==> results_postproc_abs.tex <==
\begin{table*}[ht]
\caption{Summary of the results of our experiments using a post-processing method for fairness}
\label{tab:postproc_results}
\begin{tabular}{|ccccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{4}{c|}{\textbf{Target model (under attack)}}                                                                                                               & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ Reconstructions\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Corrected\\ Reconstructions\end{tabular}}}                                                                          \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\textbf{Train Acc.}} & \multicolumn{1}{c|}{\textbf{Test Acc.}} & \multicolumn{1}{c|}{\textbf{Train Unf.}} & \multicolumn{1}{c|}{\textbf{Test Unf.}} & \multicolumn{1}{c|}{\textbf{Attacker 6}}        & \multicolumn{1}{c|}{\textbf{Attacker 7}}       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attacker 6\\ (corrected)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attacker 7\\ (corrected)\end{tabular}} \\ \hline
\multicolumn{9}{|c|}{\textbf{UCI Adult Income dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|c|}{SP}                               & \multicolumn{1}{c|}{$0.820 \pm 0.004$}   & \multicolumn{1}{c|}{$0.813 \pm 0.006$}  & \multicolumn{1}{c|}{$0.002 \pm 0.001$}   & \multicolumn{1}{c|}{$0.005 \pm 0.004$}  & \multicolumn{1}{c|}{$0.770 \pm 0.005$}          & \multicolumn{1}{c|}{$0.770 \pm 0.006$}         & \multicolumn{1}{c|}{$0.844 \pm 0.003$}                                                         & $\mathbf{0.853 \pm 0.003}$                                                \\ \hline
\multicolumn{1}{|c|}{PE}                               & \multicolumn{1}{c|}{$0.848 \pm 0.003$}   & \multicolumn{1}{c|}{$0.840 \pm 0.005$}  & \multicolumn{1}{c|}{$0.001 \pm 0.001$}   & \multicolumn{1}{c|}{$0.003 \pm 0.003$}  & \multicolumn{1}{c|}{$0.770 \pm 0.005$}          & \multicolumn{1}{c|}{$0.767 \pm 0.005$}         & \multicolumn{1}{c|}{$0.835 \pm 0.003$}                                                         & $\mathbf{0.836 \pm 0.003}$                                                \\ \hline
\multicolumn{1}{|c|}{EO}                               & \multicolumn{1}{c|}{$0.856 \pm 0.003$}   & \multicolumn{1}{c|}{$0.848 \pm 0.005$}  & \multicolumn{1}{c|}{$0.003 \pm 0.003$}   & \multicolumn{1}{c|}{$0.032 \pm 0.022$}  & \multicolumn{1}{c|}{$0.770 \pm 0.005$}          & \multicolumn{1}{c|}{$0.766 \pm 0.005$}         & \multicolumn{1}{c|}{$\mathbf{0.771 \pm 0.005}$}                                                & $0.768 \pm 0.005$                                                         \\ \hline
\multicolumn{1}{|c|}{EOdds}                            & \multicolumn{1}{c|}{$0.845 \pm 0.004$}   & \multicolumn{1}{c|}{$0.838 \pm 0.005$}  & \multicolumn{1}{c|}{$0.005 \pm 0.003$}   & \multicolumn{1}{c|}{$0.030 \pm 0.020$}  & \multicolumn{1}{c|}{$0.770 \pm 0.005$}          & \multicolumn{1}{c|}{$0.767 \pm 0.005$}         & \multicolumn{1}{c|}{$0.834 \pm 0.004$}                                                         & $\mathbf{0.835 \pm 0.005}$                                                \\ \hline
\multicolumn{9}{|c|}{\textbf{ACSPublicCoverage dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{SP}                               & \multicolumn{1}{c|}{$0.859 \pm 0.002$}   & \multicolumn{1}{c|}{$0.854 \pm 0.003$}  & \multicolumn{1}{c|}{$0.000 \pm 0.000$}   & \multicolumn{1}{c|}{$0.003 \pm 0.002$}  & \multicolumn{1}{c|}{$0.846 \pm 0.007$}          & \multicolumn{1}{c|}{$0.847 \pm 0.007$}         & \multicolumn{1}{c|}{$0.866 \pm 0.005$}                                                         & $\mathbf{0.870 \pm 0.004}$                                                \\ \hline
\multicolumn{1}{|c|}{PE}                               & \multicolumn{1}{c|}{$0.859 \pm 0.002$}   & \multicolumn{1}{c|}{$0.854 \pm 0.002$}  & \multicolumn{1}{c|}{$0.000 \pm 0.000$}   & \multicolumn{1}{c|}{$0.002 \pm 0.001$}  & \multicolumn{1}{c|}{$0.846 \pm 0.007$}          & \multicolumn{1}{c|}{$0.847 \pm 0.007$}         & \multicolumn{1}{c|}{$0.857 \pm 0.007$}                                                         & $\mathbf{0.866 \pm 0.005}$                                                \\ \hline
\multicolumn{1}{|c|}{EO}                               & \multicolumn{1}{c|}{$0.850 \pm 0.003$}   & \multicolumn{1}{c|}{$0.845 \pm 0.003$}  & \multicolumn{1}{c|}{$0.002 \pm 0.001$}   & \multicolumn{1}{c|}{$0.018 \pm 0.011$}  & \multicolumn{1}{c|}{$0.846 \pm 0.007$}          & \multicolumn{1}{c|}{$0.847 \pm 0.007$}         & \multicolumn{1}{c|}{$0.849 \pm 0.006$}                                                         & $\mathbf{0.850 \pm 0.006}$                                                \\ \hline
\multicolumn{1}{|c|}{EOdds}                            & \multicolumn{1}{c|}{$0.838 \pm 0.003$}   & \multicolumn{1}{c|}{$0.834 \pm 0.003$}  & \multicolumn{1}{c|}{$0.002 \pm 0.002$}   & \multicolumn{1}{c|}{$0.018 \pm 0.010$}  & \multicolumn{1}{c|}{$0.846 \pm 0.007$}          & \multicolumn{1}{c|}{$0.847 \pm 0.006$}         & \multicolumn{1}{c|}{$0.850 \pm 0.006$}                                                         & $\mathbf{0.851 \pm 0.006}$                                                \\ \hline
\multicolumn{9}{|c|}{\textbf{ACSIncome dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{SP}                               & \multicolumn{1}{c|}{$0.785 \pm 0.002$}   & \multicolumn{1}{c|}{$0.778 \pm 0.003$}  & \multicolumn{1}{c|}{$0.001 \pm 0.001$}   & \multicolumn{1}{c|}{$0.005 \pm 0.004$}  & \multicolumn{1}{c|}{$0.660 \pm 0.007$}          & \multicolumn{1}{c|}{$0.672 \pm 0.013$}         & \multicolumn{1}{c|}{$0.733 \pm 0.006$}                                                         & $\mathbf{0.739 \pm 0.006}$                                                \\ \hline
\multicolumn{1}{|c|}{PE}                               & \multicolumn{1}{c|}{$0.794 \pm 0.002$}   & \multicolumn{1}{c|}{$0.787 \pm 0.003$}  & \multicolumn{1}{c|}{$0.001 \pm 0.001$}   & \multicolumn{1}{c|}{$0.005 \pm 0.003$}  & \multicolumn{1}{c|}{$0.660 \pm 0.007$}          & \multicolumn{1}{c|}{$0.660 \pm 0.006$}         & \multicolumn{1}{c|}{$0.711 \pm 0.007$}                                                         & $\mathbf{0.713 \pm 0.007}$                                                \\ \hline
\multicolumn{1}{|c|}{EO}                               & \multicolumn{1}{c|}{$0.792 \pm 0.003$}   & \multicolumn{1}{c|}{$0.785 \pm 0.003$}  & \multicolumn{1}{c|}{$0.001 \pm 0.000$}   & \multicolumn{1}{c|}{$0.009 \pm 0.008$}  & \multicolumn{1}{c|}{$0.660 \pm 0.007$}          & \multicolumn{1}{c|}{$0.659 \pm 0.006$}         & \multicolumn{1}{c|}{$\mathbf{0.661 \pm 0.007}$}                                                & $0.660 \pm 0.006$                                                         \\ \hline
\multicolumn{1}{|c|}{EOdds}                            & \multicolumn{1}{c|}{$0.791 \pm 0.003$}   & \multicolumn{1}{c|}{$0.784 \pm 0.003$}  & \multicolumn{1}{c|}{$0.001 \pm 0.001$}   & \multicolumn{1}{c|}{$0.010 \pm 0.007$}  & \multicolumn{1}{c|}{$0.660 \pm 0.007$}          & \multicolumn{1}{c|}{$0.660 \pm 0.006$}         & \multicolumn{1}{c|}{$0.711 \pm 0.007$}                                                         & $\mathbf{0.712 \pm 0.007}$                                                \\ \hline
\end{tabular}
\end{table*}

==> results_target_performances_small.tex <==
\def\figwidth{0.245}%{0.245}
 %Adult Income--------------------------------
 \begin{figure*}[ht]
    \begin{center}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_1_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_3_attacker_7_accuracy.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_4_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_5_attacker_7_accuracy.pdf}
   \caption{Accuracy}
   \end{subfigure}
   \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_1_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_3_attacker_7_unfairness.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_4_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_adult_5_attacker_7_unfairness.pdf}
    \caption{Unfairness}
   \end{subfigure}
    \end{center}
    \caption{Target models performances for our experiments using the UCI Adult Income dataset}
\label{fig:target_perfs_example}
\end{figure*}

 %ACSPublicCoverage--------------------------------
 \begin{figure*}[ht]
    \begin{center}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_1_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_3_attacker_7_accuracy.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_4_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_5_attacker_7_accuracy.pdf}
   \caption{Accuracy}
   \end{subfigure}
   \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_1_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_3_attacker_7_unfairness.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_4_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSPublicCoverage_age_5_attacker_7_unfairness.pdf}
    \caption{Unfairness}
   \end{subfigure}
    \end{center}
    \caption{Target models performances for our experiments using the UCI ACSPublicCoverage dataset}
\label{fig:target_perfs_example}
\end{figure*}

 %ACSIncome--------------------------------
 \begin{figure*}[ht]
    \begin{center}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_1_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_3_attacker_7_accuracy.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_4_attacker_7_accuracy.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_5_attacker_7_accuracy.pdf}
   \caption{Accuracy}
   \end{subfigure}
   \begin{subfigure}{\textwidth}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_1_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_3_attacker_7_unfairness.pdf}
    \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_4_attacker_7_unfairness.pdf}
   \includegraphics[width=\figwidth\textwidth]{sensAttrReco_ACSIncome_race_5_attacker_7_unfairness.pdf}
    \caption{Unfairness}
   \end{subfigure}
    \end{center}
    \caption{Target models performances for our experiments using the UCI ACSIncome dataset}
\label{fig:target_perfs_example}
\end{figure*}

==> save_table_postproc.tex <==
\begin{table*}[]
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{4}{c|}{\textbf{Target model (under attack)}}                                                                                                                                                                                                                                                                                       & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ Reconstructions\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Corrected\\ Reconstructions\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Corrected\\ Reconstructions\end{tabular}}} \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Acc.\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Test\\ Acc.\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Unf.\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Test\\ Unf.\end{tabular}}} & \multicolumn{1}{c|}{\textbf{$\attackersix$}}   & \multicolumn{1}{c|}{\textbf{$\attackerseven$}}  & \multicolumn{1}{c|}{\textbf{$\attackersix$}}   & \multicolumn{1}{c|}{\textbf{$\attackerseven$}}   & \multicolumn{1}{c|}{\textbf{$\attackersix$}}             & \textbf{$\attackerseven$}             \\ \midrule
\multicolumn{11}{c}{\textbf{UCI Adult Income dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \midrule
SP                                                    & $.820 \pm .004$                                                                  & $.813 \pm .006$                                                                 & $.002 \pm .001$                                                                  & $.005 \pm .004$                                                                 & $.770 \pm .005$                              & $.770 \pm .006$                               & $.844 \pm .003$                              & \multicolumn{1}{c|}{$\mathbf{.853 \pm .003}$}  & $.841 \pm .013$                                        & $.849 \pm .014$                     \\
PE                                                    & $.848 \pm .003$                                                                  & $.840 \pm .005$                                                                 & $.001 \pm .001$                                                                  & $.003 \pm .003$                                                                 & $.770 \pm .005$                              & $.767 \pm .005$                               & $.835 \pm .003$                              & \multicolumn{1}{c|}{$\mathbf{.836 \pm .003}$}  & $.830 \pm .016$                                        & $.831 \pm .017$                     \\
EO                                                    & $.856 \pm .003$                                                                  & $.848 \pm .005$                                                                 & $.003 \pm .003$                                                                  & $.032 \pm .022$                                                                 & $.770 \pm .005$                              & $.766 \pm .005$                               & $\mathbf{.771 \pm .005}$                     & \multicolumn{1}{c|}{$.768 \pm .005$}           & $.805 \pm .029$                                        & $.804 \pm .031$                     \\
EOdds                                                 & $.845 \pm .004$                                                                  & $.838 \pm .005$                                                                 & $.005 \pm .003$                                                                  & $.030 \pm .020$                                                                 & $.770 \pm .005$                              & $.767 \pm .005$                               & $.834 \pm .004$                              & \multicolumn{1}{c|}{$\mathbf{.835 \pm .005}$}  & $.830 \pm .017$                                        & $.830 \pm .019$                     \\ \midrule
\multicolumn{11}{c}{\textbf{ACSPublicCoverage dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \midrule
SP                                                    & $.859 \pm .002$                                                                  & $.854 \pm .003$                                                                 & $.000 \pm .000$                                                                  & $.003 \pm .002$                                                                 & $.846 \pm .007$                              & $.847 \pm .007$                               & $.866 \pm .005$                              & \multicolumn{1}{c|}{$\mathbf{.870 \pm .004}$}  & $.712 \pm .034$                                        & $.720 \pm .031$                     \\
PE                                                    & $.859 \pm .002$                                                                  & $.854 \pm .002$                                                                 & $.000 \pm .000$                                                                  & $.002 \pm .001$                                                                 & $.846 \pm .007$                              & $.847 \pm .007$                               & $.857 \pm .007$                              & \multicolumn{1}{c|}{$\mathbf{.866 \pm .005}$}  & $.698 \pm .022$                                        & $.699 \pm .022$                     \\
EO                                                    & $.850 \pm .003$                                                                  & $.845 \pm .003$                                                                 & $.002 \pm .001$                                                                  & $.018 \pm .011$                                                                 & $.846 \pm .007$                              & $.847 \pm .007$                               & $.849 \pm .006$                              & \multicolumn{1}{c|}{$\mathbf{.850 \pm .006}$}  & $.675 \pm .023$                                        & $.675 \pm .024$                     \\
EOdds                                                 & $.838 \pm .003$                                                                  & $.834 \pm .003$                                                                 & $.002 \pm .002$                                                                  & $.018 \pm .010$                                                                 & $.846 \pm .007$                              & $.847 \pm .006$                               & $.850 \pm .006$                              & \multicolumn{1}{c|}{$\mathbf{.851 \pm .006}$}  & $.694 \pm .024$                                        & $.694 \pm .024$                     \\ \midrule
\multicolumn{11}{c}{\textbf{ACSIncome dataset}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
SP                                                    & $.785 \pm .002$                                                                  & $.778 \pm .003$                                                                 & $.001 \pm .001$                                                                  & $.005 \pm .004$                                                                 & $.660 \pm .007$                              & $.672 \pm .013$                               & $.733 \pm .006$                              & \multicolumn{1}{c|}{$\mathbf{.739 \pm .006}$}  & $.865 \pm .006$                                        & $.868 \pm .005$                     \\
PE                                                    & $.794 \pm .002$                                                                  & $.787 \pm .003$                                                                 & $.001 \pm .001$                                                                  & $.005 \pm .003$                                                                 & $.660 \pm .007$                              & $.660 \pm .006$                               & $.711 \pm .007$                              & \multicolumn{1}{c|}{$\mathbf{.713 \pm .007}$}  & $.853 \pm .008$                                        & $.862 \pm .007$                     \\
EO                                                    & $.792 \pm .003$                                                                  & $.785 \pm .003$                                                                 & $.001 \pm .000$                                                                  & $.009 \pm .008$                                                                 & $.660 \pm .007$                              & $.659 \pm .006$                               & $\mathbf{.661 \pm .007}$                     & \multicolumn{1}{c|}{$.660 \pm .006$}           & $.848 \pm .007$                                        & $.849 \pm .007$                     \\
EOdds                                                 & $.791 \pm .003$                                                                  & $.784 \pm .003$                                                                 & $.001 \pm .001$                                                                  & $.010 \pm .007$                                                                 & $.660 \pm .007$                              & $.660 \pm .006$                               & $.711 \pm .007$                              & \multicolumn{1}{c|}{$\mathbf{.712 \pm .007}$}  & $.855 \pm .008$                                        & $.857 \pm .008$                     \\ \bottomrule
\end{tabular}
\end{table*}

==> tentative_protection_table_large.tex <==
\begin{table*}[]
\caption{Summary of the results of our experiments using a post-processing method for fairness}
\label{tab:tentative_countermeasure_postprocessing}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{2}{c|}{\textbf{Constraint Estimation}}                                                        & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Corrected \\ (Actual Constraint)\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Corrected \\ (Estimated Constraint)\end{tabular}}} \\ \cmidrule(l){2-7} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\textbf{\%Correct Metric}} & \multicolumn{1}{c|}{\textbf{Diff. with actual tolerance}} & \multicolumn{1}{c|}{\textbf{$\attackersix$}}     & \multicolumn{1}{c|}{\textbf{$\attackerseven$}}     & \multicolumn{1}{c|}{\textbf{$\attackersix$}}       & \multicolumn{1}{c|}{\textbf{$\attackerseven$}}      \\ \midrule
\multicolumn{7}{|c|}{\textbf{UCI Adult Income dataset}}                                                                                                                                                                                                                                                                                                                                \\ \midrule
SP                                                     & $0.97$                                         & $0.004 \pm 0.004$                                         & $0.844 \pm 0.003$                                & $0.853 \pm 0.003$                                  & $0.841 \pm 0.013$                                  & $0.849 \pm 0.014$                                   \\
PE                                                     & $0.94$                                         & $0.002 \pm 0.002$                                         & $0.835 \pm 0.003$                                & $0.836 \pm 0.003$                                  & $0.830 \pm 0.016$                                  & $0.831 \pm 0.017$                                   \\
EO                                                     & $0.42$                                         & $0.016 \pm 0.009$                                         & $0.771 \pm 0.005$                                & $0.768 \pm 0.005$                                  & $0.805 \pm 0.029$                                  & $0.804 \pm 0.031$                                   \\
EOdds                                                  & $0.00$                                         & $0.003 \pm 0.003$                                         & $0.834 \pm 0.004$                                & $0.835 \pm 0.005$                                  & $0.830 \pm 0.017$                                  & $0.830 \pm 0.019$                                   \\ \midrule
\multicolumn{7}{|c|}{\textbf{ACSPublicCoverage dataset}}                                                                                                                                                                                                                                                                                                                               \\ \midrule
SP                                                     & $0.72$                                         & $0.004 \pm 0.003$                                         & $0.733 \pm 0.006$                                & $0.739 \pm 0.006$                                  & $0.712 \pm 0.034$                                  & $0.720 \pm 0.031$                                   \\
PE                                                     & $0.77$                                         & $0.004 \pm 0.003$                                         & $0.711 \pm 0.007$                                & $0.713 \pm 0.007$                                  & $0.698 \pm 0.022$                                  & $0.699 \pm 0.022$                                   \\
EO                                                     & $0.69$                                         & $0.007 \pm 0.005$                                         & $0.661 \pm 0.007$                                & $0.660 \pm 0.006$                                  & $0.675 \pm 0.023$                                  & $0.675 \pm 0.024$                                   \\
EOdds                                                  & $0.00$                                         & $0.003 \pm 0.003$                                         & $0.711 \pm 0.007$                                & $0.712 \pm 0.007$                                  & $0.694 \pm 0.024$                                  & $0.694 \pm 0.024$                                   \\ \midrule
\multicolumn{7}{|c|}{\textbf{ACSIncome dataset}}                                                                                                                                                                                                                                                                                                                                       \\ \midrule
SP                                                     & $0.99$                                         & $0.003 \pm 0.002$                                         & $0.866 \pm 0.005$                                & $0.870 \pm 0.004$                                  & $0.865 \pm 0.006$                                  & $0.868 \pm 0.005$                                   \\
PE                                                     & $1.00$                                         & $0.002 \pm 0.002$                                         & $0.857 \pm 0.007$                                & $0.866 \pm 0.005$                                  & $0.853 \pm 0.008$                                  & $0.862 \pm 0.007$                                   \\
EO                                                     & $0.36$                                         & $0.009 \pm 0.004$                                         & $0.849 \pm 0.006$                                & $0.850 \pm 0.006$                                  & $0.848 \pm 0.007$                                  & $0.849 \pm 0.007$                                   \\
EOdds                                                  & $0.00$                                         & $0.002 \pm 0.002$                                         & $0.850 \pm 0.006$                                & $0.851 \pm 0.006$                                  & $0.855 \pm 0.008$                                  & $0.857 \pm 0.008$                                   \\ \cmidrule(r){1-1} \cmidrule(l){4-7} 
\end{tabular}
\end{table*}
